Transformations between Composite and Visitor implementations in Java

Basic automated refactoring operations can be chained to perform complex structure transformations. This is useful for recovering the initial architecture of a source code which has been degenerated with successive evolutions during its maintenance lifetime. This is also useful for changing the structure of a program so that a maintenance task at hand becomes modular when it would be initially crosscutting. We focus on programs structured according to Composite and Visitor design patterns, which have dual properties with respect to modularity. We consider a refactoring-based round-trip transformation between these two structures and we study how that transformation is impacted by four variations in the implementation of these patterns. We validate that study by computing the smallest preconditions for the resulting transformations. We also automate the transformation and apply it to JHotDraw, where the studied variations occur.

==> Variation_FACADE_RETOUR.tex <==


  Starting from the target structure shown above, we remark that the recursive call to \textit{accept} is referring to the \textit{accept} method declared 
in the interface \xcode{Figure}. This influences the backward transformation as follows: 
\begin{itemize}
 \item In order to get back the recursive call of the delegator \xcode{print()}, we have to make a downcast to the recursive call which 
is referring to \xcode{Figure} 
 before applying step~\ref{visitor-composite-algo:fold} (step~\ref{visitor-composite-algo:fold}.D).

 \item Delete the method that was an \textit{accept} method before from the interface \xcode{Figure}.
 \item To get back the initial program, we delete the downcast (step\ref{visitor-composite-algo:pushdown-m}.D).
\end{itemize}


\noindent\begin{boxedminipage}{\columnwidth}
\begin{enumerate}[XXX.X]
 

\item[\ref{visitor-composite-algo:fold}.D] ForAll m in $\mathbb{M}$, c in $\mathbb{C}$ do\\ \tab \tab
  \textbf{IntroduceDownCast}(c,m,S)  \hfill (before~\ref{visitor-composite-algo:fold})

\item[\ref{visitor-composite-algo:pushdown-m}.D]
       ForAll m in $\mathbb{M}$ do\\ \tab \tab 
         \textbf{PushDownAll}(I,\auxname{m}) \\ %\tab \tab
%
       ForAll c in $\mathbb{C}$, m in $\mathbb{M}$ in  do \\ \tab \tab
           \textbf{DeleteDownCast}(c,m)  \hfill \hfill (after~\ref{visitor-composite-algo:fold})
\end{enumerate}

\end{boxedminipage}\\



The generated preconditions don't take into account the transformation with down cast. We remark the absence of the preconditions $\mathsf{IsRecursiveMethod}(Group,print)$ and $\mathsf{IsRecursiveMethod}(Group,show)$ 
form the minimum preconditions of this transformation. This is due to the non application of 
the operation \emph{InlineMethodInvocations} of step~\ref{algo-composite-visitor:inline-methods} which is used to inline recursive calls of business methods 
to create later the recursive call of the \textit{accept} method.

